RigNeRF: Fully Controllable Neural 3D Portraits

Volumetric neural rendering methods, such as neural radiance fields (NeRFs), have enabled photo-realistic novel view synthesis. However, in their standard form, NeRFs do not support the editing of objects, such as a human head, within a scene. In this work, we propose RigNeRF, a system that goes beyond just novel view synthesis and enables full control of head pose and facial expressions learned from a single portrait video. We model changes in head pose and facial expressions using a deformation field that is guided by a 3D morphable face model (3DMM). The 3DMM effectively acts as a prior for RigNeRF that learns to predict only residuals to the 3DMM deformations and allows us to render novel (rigid) poses and (non-rigid) expressions that were not present in the input sequence. Using only a smartphone-captured short video of a subject for training, we demonstrate the effectiveness of our method on free view synthesis of a portrait scene with explicit head pose and expression controls. The project page can be found here: http://shahrukhathar.github.io/2022/06/06/RigNeRF.html

==> cvpr22/teaser.tex <==
\centering
\includegraphics[width=0.95\linewidth]{cvpr22/teaserimg.pdf}
     \figcaption{{Our method, \MethodName, enables full control of head-pose and facial expression of a human portrait using a 3DMM-guided deformable neural radiance field. With a short portrait video for training, \MethodName can reanimate the subject with arbitrary (a) head-pose and (b) facial expressions. It also allows controllable viewpoints of the 3D scene (c).  Naturally \MethodName can be used to transfer facial animation from a driving video sequence to the 3D portraits faithfully (d).%
    }}
